Variable importance measure for spatial machine learning models with application to air pollution exposure prediction

Exposure assessment is fundamental to air pollution cohort studies. The objective is to predict air pollution exposures for study subjects at locations without data in order to optimize our ability to learn about health effects of air pollution. In addition to generating accurate predictions to minimize exposure measurement error, understanding the mechanism captured by the model is another crucial aspect that may not always be straightforward due to the complex nature of machine learning methods, as well as the lack of unifying notions of variable importance. This is further complicated in air pollution modeling by the presence of spatial correlation. We tackle these challenges in two datasets: sulfur (S) from regulatory United States national PM2.5 sub-species data and ultrafine particles (UFP) from a new Seattle-area traffic-related air pollution dataset. Our key contribution is a leave-one-out approach for variable importance that leads to interpretable and comparable measures for a broad class of models with separable mean and covariance components. We illustrate our approach with several spatial machine learning models, and it clearly highlights the difference in model mechanisms, even for those producing similar predictions. We leverage insights from this variable importance measure to assess the relative utilities of two exposure models for S and UFP that have similar out-of-sample prediction accuracies but appear to draw on different types of spatial information to make predictions.

==> method-old.tex <==
%%%%%%%%%%%
\section{Leave-One-Out Evaluation of Quantile-Level Contrasts }
\label{sec:method}
%%%%%%%%%%%

%\sccomm{Question to consider: for what classes of spatial models does our approach work;
%e.g. spatial models where spatial correlation are explicitly captured by a smoothing term? (any better high-level description for such class of models?)
%For such models, our LOO approach is ``fast'' (in the sense that the whole model does not need to be re-fit and the procedure can be parallelized)}

We now introduce a variable importance measure that is applicable to additive models taking the form of (\ref{equ:meanmod}) as described in Section~\ref{sec:model}. This leave-one-out approach is based on the change in predictions across different user-specified quantiles $q_1, \ldots, q_m$ for each covariate, evaluating at each location $s_1, \ldots, s_n$ one at a time.
For the mean (i.e. each $f_k$) and error (i.e. each $\nu_k$) components, the majority amount of computation typically comes from estimating the former, and once a mean model $f_k$ is fitted, changing the covariate values at one location does not affect the mean predictions $\hat f_k$ at other locations. 
Therefore, the key idea of the proposed approach is to reuse the fitted mean model across all locations, but re-fit the error component in a leave-one-out manner. 
We write $\hat F_{X_j}(x_j), j = 1, \ldots, p$ as the empirical cumulative distribution function (CDF) of the $j$th covariate, and $\boldsymbol s_{-i}$ as the set of all locations except the $i$th one. 

Suppose we have a fitted model
\[
    g\left(\hat\mu(s)\right) = \sum_{i=1}^K \left[\hat f_k(X(s)) + \hat\nu_k(s) \right]
\]
from observations $\{(X(s_i), Y(s_i))\}_{i=1}^n$. Then for the $j$th covariate, at the $l$th quantile $q_l$ of interest, within the $k$th sub-model $\hat f_k$ and for the $i$th location $s_i$, one could obtain the fitted means $\hat f_k\left(X(\boldsymbol s_{-i})\right)$ at all other locations, and calculate the predicted mean as
\[
    \hat\zeta_{k}^{j,l}(s_{i}) := \hat f_k\left(X_1(s_{i}), \ldots, \hat F_{X_j}^{-1}(q_l), \ldots, X_p(s_{i})\right)
\]
for location $i$. In plain words, this is the predicted mean at $s_i$ with the $j$th covariate replaced by its $q_l$-th quantile across $s_1, \ldots, s_n$. 
%\begin{equation}
%    \hat\zeta_{k}^{j,l}(s_{i'}) := 
%    \begin{cases}
%        \hat f_k\left(X_1(s_{i'}), \ldots, \hat F_{X_j}^{-1}(q_l), \ldots, X_p(s_{i'})\right), \quad i' = i\\
%        \hat f_k\left(X(s_{i'})\right), \quad i'\neq i.
%    \end{cases}
%    \label{equ:fittedmeans}
%\end{equation}
%In plain words, the predicted mean at the $i$th location is calculated with the $j$th covariate replaced by its $q_l$-th quantile, while those at all other locations are simply the fitted means.
Next, we re-fit the $k$th error component with the predicted means $\hat f_k\left(X(\boldsymbol s_{-i})\right)$ along with observations $\left(X({\boldsymbol s_{-i}}), Y({\boldsymbol s_{-i}})\right)$, leaving out the $i$th site. Denoting the resulting model as $\hat\nu_{(-i),k}^{j,l}(s)$, the leave-one-out approach yields the linear predictor
\begin{equation}
    \hat\eta_{k}^{j,l}(s_i) := \hat\zeta_{k}^{j,l}(s_i) + \mathbb E\left[\hat\nu_{(-i), k}^{j, l}(s_i)\mid Y(\boldsymbol s_{-i}), \hat f_k\left(X(\boldsymbol s_{-i})\right)\right]
    \label{equ:linear-pred}
\end{equation}
for location $i$, which is what the model would predict if the $j$th covariate of the $i$th data point were replaced by the $q_l$-quantile, and if the error component were fitted without the $i$th data point, while keeping everything else intact.

Re-doing this for all $i$, we obtain a sequence of linear predictors of the form (\ref{equ:linear-pred}). Aggregating across each sub-model (each $k$) and location (each $i$) finally leads to the averaged leave-one-out predictions at the $q_l$-th quantile for covariate $j$:
\begin{equation}
    \bar\mu_{j,l} := g^{-1}\left(\frac{1}{n} \sum_{i=1}^n \sum_{k=1}^K \hat\eta_{k}^{j,l}(s_i) \right).
\end{equation}

For each $j$, the trajectory $\bar\mu_{j,1}, \ldots, \bar\mu_{j,m}$ reflects how the predictions, on average, vary across different quantiles of covariate $X_j$, which serves as an intuitive measure of the contribution of this covariate on the predicted outcome. This procedure could easily be parallelized to facilitate computation. Algorithm~\ref{algo:varimp} presents the described procedure in detail. 

\RestyleAlgo{boxruled}
% \LinesNumbered
\SetAlgoNoLine
\begin{algorithm}[!ht]
  \caption{Leave-one-out variable importance\label{algo:varimp}}
  Set quantile levels $q_1, \ldots, q_m \in [0, 1]$, and of interest. Input the data $(X_{n\times p}, Y_{n\times 1})$ and a trained model 
  \[
    g\left(\hat\mu(s)\right) = \sum_{k=1}^K \left[\hat f_k(X(s)) + \hat\nu_k(s) \right]
  \]\;
        
    \For{$i = 1, \ldots, n$}{
        \For{$k = 1, \ldots, K$}{
        Re-fit a covariance model with $(X_{-i,\cdot}, Y_{-i})$ conditioning on the mean model $\hat f_k(\boldsymbol s_{-i})$, denoted as $\hat\nu_{(-i),k}(s)$\;
        
            \For{$j = 1, \ldots, p$}{
                \For{$l = 1, \ldots, m$}{
                    Calculate the fitted mean at all but the $i$th location as $\hat\zeta_k^{j,l}(\boldsymbol s_{-i}):=\hat f_k(X(\boldsymbol s_{-i}))$\;
                    
                    Replace the $i$th observation of the $j$th covariate, $X_{ij}$, with the $q_l$-th sample quantile $\hat F_{X_j}^{-1}(q_l)$:
                    \[
                        \tilde X_{i\cdot} := \left(X_1(s_{i}), \ldots, \hat F_{X_j}^{-1}(q_l), \ldots, X_p(s_{i})\right)
                    \]
                    
                    Calculate the predicted mean at the $i$th location as $\hat\zeta_k^{j,l}(s_i):= \hat f_k(\tilde X_{i\cdot})$\;
                    
                    % Re-fit a covariance model with $(X_{-i,\cdot}, Y_{-i})$ conditioning on the mean model $\hat\zeta_k^{j,l}(s)$, denoted as $\hat\nu_{(-i),k}^{j,l}(s)$\;
                    Evaluate the covariance term for location $i$ from the fitted model $\hat\nu_{k}^{j,l}(s_i) := \mathbb E \left[\nu_{(-i), k}(s_i)\mid Y(\boldsymbol s_{-i}), \hat f_k\left(X(\boldsymbol s_{-i})\right)\right]$\;
                    % $\hat\nu_{k}^{j,l}(s_i) := \mathbb E \left[\nu_{(-i), k}^{j, l}(s_i)\mid Y(\boldsymbol s_{-i}), \hat f_k\left(X(\boldsymbol s_{-i})\right)\right]$\;
                    
                    Calculate the linear predictor for location $i$ as $\hat\eta_{k}^{j,l}(s_i) := \hat\zeta_{k}^{j,l}(s_i) + \hat\nu_{k}^{j,l}(s_i)$\;
                    
                    Calculate the averaged leave-one-out predictions $\bar\mu_{j,l} := g^{-1}\left(\frac{1}{n} \sum_{i=1}^n \sum_{k=1}^K \hat\eta_{k}^{j,l}(s_i) \right)$\;
                }
            }
        }
    }
    \KwResult{Output averaged leave-one-out predictions $\bar\mu_{j,l}$ for each $j = 1, \ldots, p$, and $l = 1, \ldots, m$. }
\end{algorithm}

==> models.tex <==
%%%%%%%%%%%
\section{Spatial Prediction}
\label{sec:model}
%%%%%%%%%%%

Before introducing the proposed variable importance measure, we describe a broad class of spatial prediction models to which such measure is applicable.
Consider a class of models where an outcome $Y(s)$, indexed by location $s\in \Omega$, is modeled via an additive mean surface taking the form of

\begin{equation}
    g(\mu(s)) = \sum_{k=1}^K [f_k\left(X(s)\right) + \nu_k(s)]
    \label{equ:meanmod}
\end{equation}
where $g(\cdot)$ is a link function, $X(s)$ represents the covariates, each $\nu_k(s)$ represents the correlated error term, and each $f_k(\cdot)$ is an unknown function within some function class $\mathcal F$. The indexing $k$ allows for application to ensemble learning methods.
% Note that when $\nu(s)$ is non-degenerate, this corresponds to a doubly-stochastic process \citep{cox1955some} where the mean surface relies on the realization of a random error field. 
As an example, when $g$ is the logarithm link function and $\nu(s)$ is a correlated Gaussian process, $\mu(s)$ is the underlying intensity of a doubly-stochastic Poisson process, also known as the Cox process \citep{cox1955some, serfozo1972conditional, bremaud1981point}; when $g$ is the identity link and $\nu(s)$ is a correlated Gaussian process, $\mu(s)$ models the surface of a continuous outcome, e.g. a universal kriging model if $f$ is linear.

A spatial ML model often learns about each $f_k$ under some assumed restrictions on $\mathcal F$, and $\nu_k(s)$ under parametric or structural assumptions. Once a model (\ref{equ:meanmod}) is fitted at a set of training sites $s_{\text{trn}}$, predictions at the test sites $ s_{\text{tst}}$ can be made via
\[
    \hat Y( s_{\text{tst}}) = g^{-1} \left(\sum_{k=1}^K \left\{ \hat f_{k}(X( s_{\text{tst}})) + \mathbb E \left[ \nu_k (s_{\text{tst}}) \mid Y(s_{\text{trn}}), \hat f_k(s_{\text{trn}}) \right] \right\}\right),
\]
where the conditional expectation $\mathbb E \left[ \hat\nu_k (s_{\text{tst}}) \mid Y(s_{\text{trn}}), \hat f_k(s_{\text{trn}}) \right]$ represents the smoothing of residuals \sccomm{via the fitted covariance model $\hat\nu_k(s)$} at the training sites. When $g$ is identity and each $\nu_k$ is assumed to be a correlated Gaussian random field with covariance $\Sigma(\theta)$, for example, the model predicts
\begin{equation*}
    \hat\nu_k (s_{\text{tst}}) := \mathbb E \left[ \nu_k (s_{\text{tst}}) \mid Y(s_{\text{trn}}), \hat f_k(s_{\text{trn}}) \right] = \Sigma(\hat\theta)_{\text{tst,trn}} \left[\Sigma(\hat\theta)_{\text{trn,trn}} \right]^{-1} \left(Y(s_{\text{trn}}) - \hat f_k(s_{\text{trn}})
    \right).
\end{equation*}

As an illustration and for concreteness of our following discussions, we revisit two the models introduced in Section~\ref{subsec:data-pred} for an observed continuous outcome $Y_{n\times 1}$, with identity $g(\cdot)$ and potentially high-dimensional covariates $X_{n\times p}$, and describe how they fit into this framework.
One model is UK-PLS, which \sccomm{has $k = 1$ and} first conducts PLS and extracts the first $l$ ($1\le l \le p$) components of $X$ by finding a decomposition of $X$
\begin{align*}
    T_{n\times l} := X_{n\times p} H_{p\times l}
\end{align*}
such that the covariance between $T$ and $Y$ is maximized. The number $l$ of components to use can be selected via cross-validation. In the second step, a universal kriging model
\begin{align*}
    Y_{n\times 1} &= T_{n\times l}\beta_{l\times 1} + \nu_{n\times 1} \\
    \nu_{n\times 1} &\sim \text{Normal}(0, \Sigma(\theta))
\end{align*}
where $\theta$ are covariance parameters (e.g. the nugget, partial sill and range, see \citet{cressie2015statistics}) which can be solved jointly with $\beta$ via maximum likelihood. With $\hat H_{p\times l}, \hat\beta, \hat\theta$ estimated from the model, for $m$ new (test) locations with covariate values $X^*_{m\times p}$, the outcome $Y^*$ can be predicted as
\begin{align*}
    \hat Y^* = X^*\hat H\hat\beta + \mathbb E_{\theta}[\nu^*\mid \nu]
    = X^*\hat H\hat\beta + \tilde\Sigma_{12}(\hat\theta) \tilde\Sigma_{22}^{-1}(\hat\theta) 
    \left( Y - T\hat\beta \right)
\end{align*}
where $\tilde\Sigma_{(m+n)\times (m+n)}(\hat\theta)$ is the covariance matrix induced by the distances between all training and test locations, partitioned as
\begin{equation}
    \tilde\Sigma(\hat\theta) = \begin{bmatrix}
        \tilde\Sigma_{11}^{(m\times m)} & \tilde\Sigma_{12}^{(m\times n)}\\
        \tilde\Sigma_{21}^{(n\times m)} & \tilde\Sigma_{22}^{(n\times n)}
    \end{bmatrix}
    \label{equ:Sig-partition}
\end{equation}
based on the training and test indices. %\sccomm{Algorithm? Or are these notations explicit enough?}

The second example is the spatial random forest algorithm proposed by \citet{wai2020random} solved via pseudo-likelihood (SpatRF-PL). It \sccomm{is an ensemble model (i.e. $k > 1$) which} specifies 
\begin{equation}
    \hat\mu(s) := \sum_{k=1}^K \hat\mu_k(s) := \sum_{k=1}^K \left[ \hat f_k(X(s)) + \hat\nu_k(s) \right]
    \label{equ:spatrf}
\end{equation}
where each $f_k$ is a regression tree, and each $\nu_k$ could be modeled via common spatial smoothing methods such as kriging or regression splines \citep{friedman1991multivariate, wood2003thin}. %Parameters for the two components (tree splitting design matrix and weights, along with smoothing parameters) are estimated jointly. 
With a kriging model, for each $k$, a spatially adjusted tree can be built by solving the optimization problem resulting from profile likelihood, assuming normally distributed spatial error terms:
\begin{align}
    \notag \arg\max_{\theta_k} & \left[-\frac{1}{2}\log\lvert\Sigma(\theta_k)\rvert
    -\frac{1}{2}\left(Y - \hat f_k(X\mid \Sigma(\theta_k)) \right)^\top \Sigma^{-1}(\theta_k)\left(Y - \hat f_k(X\mid \Sigma(\theta_k)) \right)
    \right]\\
    & \text{s.t. } \hat f_k(X\mid\Sigma(\theta_k)) = \arg\min_{f_k(X\mid\Sigma(\theta_k))}
    \left(Y -  f_k(X\mid \Sigma(\theta_k)) \right)^\top \Sigma^{-1}(\theta_k)\left(Y -  f_k(X\mid \Sigma(\theta_k)) \right).
    \label{equ:spat-tree}
\end{align}

And likewise, predictions at test locations can be made via
\[
    \hat Y^* = \sum_{k=1}^K \left[
        \hat f_k(X^*) + \mathbb E_{\hat\theta_k} \left(\nu^*\mid \nu\right)
    \right]
    = \sum_{k=1}^K \left[
        \hat f_k(X^*) + \tilde\Sigma_{12}(\hat\theta_k) \tilde\Sigma_{22}^{-1}(\hat\theta_k) 
    \left( Y - \hat f_k(X) \right)
    \right]
\]
with $\tilde\Sigma$ defined identically as (\ref{equ:Sig-partition}).

==> sim.tex <==
%%%%%%%%%%%
\section{Illustration with Synthetic Data}
\label{sec:sim}
%%%%%%%%%%%

To further illustrate how the proposed variable importance measure performs in comparison to the true mechanism, we present a variable importance analysis with synthetic data generated with the same covariates as the national study. We generated a continuous outcome with 5 active predictors
\begin{itemize}
    \item Distance to A1 road
    \item Population density
    \item Annual median NDVI, buffer size 1km
    \item Land use: mixed urban, buffer size 15km
    \item Land use: residential, buffer size 15km
\end{itemize}
which were all scaled and centered, except population density and mixed urban land use which were shifted to be non-negative. The mean model was given by
\begin{align*}
    \mathbb E(Y\mid X) = & -0.5\times \text{distance to A1 road} + 0.2\times \text{population density}^2 - 1\times \text{annual median NDVI}\\
    & + 0.5\times\sqrt{\text{mixed urban land use}} + 0.5\times \text{residential land use}\\
    & -0.25\times \text{distance to A1 road}\times\text{annual median NDVI}. 
\end{align*}

The correlated error term was given by an exponential model with scale and range parameter equal to 4 and 2.5 respectively, where the unit of distance was 1000km. The uncorrelated errors were generated from a standard Gaussian distribution. With this setup, the variances of each component (mean, partial sill and nugget) in the outcome were 2.21, 1.07 and 1.02 respectively, so that we roughly have a 2:1:1 variance decomposition of the outcome, as visualized in Figure~\ref{fig:y_decomp}.

\begin{figure}
    \centering
    \includegraphics[width=17cm]{figures/Y_decomp.jpeg}
    \caption{Decomposition of the synthetic outcome}
    \label{fig:y_decomp}
\end{figure}

Table~\ref{tab:r2_synthetic} compares the predictive performance of different models on the generated data, where we observe that models capturing the mean (RF) or correlation (TPRS) only have the lowest accuracy, and UK-PLS which only captures linear relationship has worse performance comparing to more flexible models (two-step models or Spatial RF).

Figure~\ref{fig:varimp_syn} shows the proposed variable importance measure together with the maximum absolute correlation between each predictor and each truly active predictor. 
Due to the autocorrelation between predictors, it is unlikely that any variable importance measure would exactly recover the true predictor contributions. 
Instead, a reasonably good measure would highlight predictors that are highly correlated the truly active ones, which would explain the mechanism well enough for practical purposes such as prediction. Our method achieves this, as reflected by the observation that predictors found to have high contribution in the first three panels are either the true ones (e.g. annual median NDVI) or highly correlated with at least one truly active predictor (e.g. transportation land use, which has a maximum absolute correlation above 0.75 with the true predictors as seen from the last panel).
\sccomm{I'll come back later to edit the y-axis labels...}
% Through this variable importance measure, both UK-PLS and Spatial RF identified the truly active predictors, despite lower magnitude due to autocorrelation between predictors. 

\begin{table}[ht]
\centering
\begin{tabular}{@{}lllllll@{}}
\toprule
UK-PLS & RF   & TPRS & RF-TPRS & TPRS-RF & SpatRF (PL) & SpatRF (NP) \\ \midrule
0.62   & 0.61 & 0.32 & 0.69    & 0.67    & 0.72        & 0.72        \\ \bottomrule
\end{tabular}
\caption{Cross-validated $R^2$ for each method on synthetic data}
\label{tab:r2_synthetic}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=17cm]{figures/syn_varimp_full.jpeg}
    \caption{First three columns: variable importance of spatial RF and UK-PLS; last column: maximum absolute correlation between each predictor and the 5 truly active predictors}
    \label{fig:varimp_syn}
\end{figure}

Figure~\ref{fig:vim_corr} further reflects the fact that both UK-PLS and spatial RF tend to allocate the contribution of the true predictors onto others highly correlated with them, and conversely, only the predictors that are highly correlated with the true ones could be found to have a meaningful contribution in the model. Again, the plot also suggests that the greedy-based tree building algorithm tends to favor more parsimonious model when autocorrelation is present among predictors.

\begin{figure}
    \centering
    \includegraphics[width=16.5cm]{figures/syn_scattered_corr.jpeg}
    \caption{Distribution of variable importance versus correlation with truly active predictors. The $x$-axis is the maximum absolute correlation between each predictor across all 5 active predictors.}
    \label{fig:vim_corr}
\end{figure}
